Root systems and generalized associahedra

These lecture notes for the IAS/Park City Graduate Summer School in Geometric Combinatorics (July 2004) provide an overview of root systems, generalized associahedra, and the combinatorics of clusters. Lectures 1-2 cover classical material: root systems, finite reflection groups, and the Cartan-Killing classification. Lectures 3-4 provide an introduction to cluster algebras from a combinatorial perspective. Lecture 5 is devoted to related topics in enumerative combinatorics.

==> pcmslmod14fr.tex <==
% Make sure author names get written to table of contents
% We are assuming that \part* is always used, never the unstarred form!

\makeatletter

\def\@spart#1{%\addcontentsline{toc}{part}{#1}%
\def\thispart{#1}
  \begingroup\huge\bfseries
   \vspace*{8pc}%
   \ifodd\c@page\raggedleft\else\raggedright\fi
   #1\endgraf
  \endgroup}

\def\pauth#1{%
\addcontentsline{toc}{part}{#1, \thispart}%
{\raggedleft\vspace*{2pc}%
        \LARGE\bfseries\noindent
        #1\endgraf\vfill\newpage}}
\makeatother

% Paragraph is not defined in the table of contents routines in the
% style file

\makeatletter
\def\l@paragraph{\@tocline{5}{0pt}{1pc}{7pc}{}}
\let\tocparagraph\tocsection
\makeatother

% Change the definition of \tableofcontents, so that it creates a .toc
% file but doesn't write a table of contents into the individual
% lecture series.

\makeatletter
\def\@starttoc#1#2{%
%  \begingroup
%  \let\secdef\@gobbletwo \chapter
%  \let\@secnumber\@empty % for \@tocwrite and \chaptermark
%  \ifx\contentsname#2%
%  \else \@tocwrite{chapter}{#2}\fi
%  \typeout{#2}\@xp\chaptermark\@xp{#2}%
%  \@makeschapterhead{#2}\@afterheading
  \makeatletter
%  \@input{\jobname.#1}%
  \if@filesw
    \@xp\newwrite\csname tf@#1\endcsname
    \immediate\@xp\openout\csname tf@#1\endcsname \jobname.#1\relax
  \fi
%  \global\@nobreakfalse \endgroup
%  \newpage
\makeatother
}
\makeatother

% Undo Dan's change to copyright year, since there is sometimes a delay

\makeatletter
\def\@setcopyright{%
%  \let\copyrightyear\currentyear             % DF
  \insert\copyins{\hsize\textwidth
    \parfillskip\z@ \leftskip\z@\@plus.9\textwidth
    \fontsize{6}{7\p@}\normalfont\upshape
    \everypar{}%
    \vskip-\skip\copyins \nointerlineskip
    \noindent\vrule\@width\z@\@height\skip\copyins
    \copyright\copyrightyear\ Sergey Fomin and Nathan Reading\par
    \kern\z@}%
}
\makeatother

% Data for volume 14

\def\currentvolume{14}
\def\currentyear{2004}
\def\copyrightyear{2007}

